The chemical yields of stars in the range 9-15 Msun

In Limongi et al. (2024) we presented and discussed the main evolutionary properties and final fate of stars in the mass range 7-15 Msun. The evolutions of those models were computed by means of a medium size nuclear network that guaranteed a proper calculation of the nuclear energy generation and hence a good modeling of the physical evolution of these stars. In the present paper, we extend this study by computing the detailed chemical yields of stars in the mass range 9-15 Msun, i.e., those stars that explode as core collapse supernovae (CCSNe). The explosive nucleosynthesis is then computed in the framework of the thermal bomb induced explosion by means of the HYPERION code (Limongi and Chieffi 2020). We find that: (1) the yields of the intermediate mass elements (i.e., O to P) show a steep decrease as the inital mass decreases; (2) the yields of s-weak component, i.e., those produced by the slow neutron captures from Ga to to the first neutron closure shell, decrease almost linearly as a function of the initial mass with respect to the ones produced by the more massive stars; (3) the global contribution of the stars in the mass range 9.22-13 Msun to the yields of a generation of massive stars averaged over a standard initial mass function is negligible for essentially all the isotopes. In spite of this, however, the models of stars in this mass range can be fundamental to interpret the observations of specific supernovae.

==> tabmainprop2.tex <==
%\floattable
\startlongtable
\begin{deluxetable*}{lccccccc}\label{tab_main_prop}
%\centerwidetable
%\tablewidth{0pt}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
%\movetableright=1cm
\tablecolumns{8}
\tablecaption{Main properties of the computed models}
\tablehead{\colhead{} & \colhead{9.22} & \colhead{9.50} & \colhead{10.00} & \colhead{11.00} & \colhead{12.00} & \colhead{13.00} & \colhead{15.00} } 
\startdata    
\cutinhead{ H burning}                                       
  $\rm M_{CC}$              & 3.33     & 3.50    & 3.71    & 4.19    & 4.74    & 5.24    & 6.39     \\   
  $\rm t$                   & 2.91(7)  & 2.76(7) & 2.50(7) & 2.11(7) & 1.83(7) & 1.62(7) & 1.31(7)  \\   
  $\rm M_{He }$             & 1.66     & 1.76    & 1.90    & 2.19    & 2.54    & 2.93    & 3.70     \\   
  $\rm M_{tot}$             & 9.18     & 9.42    & 9.96    & 10.91   & 11.89   & 12.88   & 14.89    \\   
\cutinhead{ He burning}                                                                 
  $\rm M_{CC}$              & 1.09     & 1.15    & 1.23    & 1.49    & 1.74    & 2.03    & 2.69     \\    
  $\rm t$                   & 2.50(6)  & 2.36(6) & 2.12(6) & 1.74(6) & 1.48(6) & 1.27(6) & 1.01(6)  \\   
  $\rm ^{12}C$              & 0.453    & 0.451   & 0.448   & 0.434   & 0.423   & 0.412   & 0.390    \\   
  $\rm M_{CO}$              & 1.08     & 1.15    & 1.23    & 1.48    & 1.74    & 2.03    & 2.69     \\   
  $\rm M_{He}$              & 2.51     & 2.56    & 2.72    & 3.10    & 3.49    & 3.90    & 4.77     \\   
  $\rm M_{CE}$              & 4.09     & 3.41    & 3.64    & 3.87    & 4.16    & 4.61    & 5.32     \\   
  $\rm M_{tot}$             & 8.89     & 8.90    & 9.61    & 10.39   & 11.28   & 12.15   & 13.93     \\   
\cutinhead{ Quantities at Carbon Ignition}                                                            
%  Model                    &   10200   & 8100  & 9200  & 9100  & 9000  & 8900  &   8900    \\   
  $\rm Log(T_{ign})$        &    8.831  & 8.846 & 8.833 & 8.834 & 8.841 & 8.843 &    8.854  \\   
  $\rm Log(\rho_{ign})$     &    6.133  & 6.115 & 6.096 & 5.881 & 5.725 & 5.583 &    5.381  \\   
  $\rm \psi_{ign}$          &    2.450  & 2.250 & 2.272 & 1.412 & 0.832 & 0.374 &    -0.25  \\     
  $\rm M_{ign}$             &    0.082  & 0.022 & 0.000 & 0.000 & 0.000 & 0.000 &    0.000  \\   
  $\rm M_{CO}$              &    1.299  & 1.337 & 1.388 & 1.590 & 1.800 & 2.066 &    2.685  \\    
  $\rm M_{He}$              &    2.545  & 2.567 & 2.717 & 3.098 & 3.486 & 3.905 &    4.777  \\   
  $\rm M_{CE}$              &    2.548  & 2.646 & 2.817 & 3.218 & 3.627 & 4.065 &    4.985  \\   
  $\rm M_{tot}$             &    8.828  & 9.019 & 9.537 & 10.357& 11.212&12.017 &   13.684  \\
\cutinhead{ Quantities at Neon Ignition}                                                            
%                                  9.22      9.5      10.00     11.00     12.00     13.00     15.00
%%  Model                         38500   & 26800   &  15100  & 14000   & 13400   & 13200   & 12750   \\   
  $\rm ^{12}C    $              & 0.004   & 0.003   & 0.000   & 0.000   & 0.000   & 0.000   & 0.000   \\   
  $\rm M_{C}$                   & 0.000   & 0.000   & 0.000   & 0.000   & 0.000   & 0.000   & 0.000   \\   
  $\rm Log(T_{ign})$            & 9.138   & 9.174   & 9.179   & 9.160   & 9.166   & 9.167   & 9.145   \\   
  $\rm Log(\rho_{ign})$         & 7.443   & 7.393   & 7.324   & 7.279   & 7.227   & 7.197   & 6.990   \\   
  $\rm \psi_{ign}$              & 6.653   & 7.753   & 5.216   & 5.193   & 4.790   & 4.603   & 3.709   \\     
  $\rm M_{ign}$                 & 0.932   & 0.678   & 0.571   & 0.200   & 0.058   & 0.000   & 0.000   \\   
  $\rm M_{ONe}$                 & 1.35278 & 1.39464 & 1.44708 & 1.58160 & 1.73310 & 1.96181 & 2.44923 \\
  $\rm M_{CO}$                  & 1.36596 & 1.41083 & 1.47756 & 1.69028 & 1.87176 & 2.16383 & 2.76339 \\   
  $\rm M_{He}$                  & 1.57790 & 1.63675 & 2.71881 & 3.10040 & 3.48811 & 3.90071 & 4.77717 \\   
  $\rm M_{CE}$                  & 1.57879 & 1.63817 & 2.73556 & 3.16664 & 3.69772 & 4.02512 & 4.97346 \\   
  $\rm M_{tot}$                 & 8.754   & 9.006   & 9.42941 & 10.2382 & 11.0858 & 11.9091 & 13.6103 \\   
\cutinhead{ Quantities at Si-S Ignition}                                                            
%                                  9.22      9.5         10.00     11.00     12.00     13.00    15.00
%%%%  Model                       178400    231200       48000    53200     25500     23500     20100
 $\rm Log(T_{ign})$             & 9.509    & 9.471     &  9.473  & 9.475   & 9.494   & 9.530   & 9.513    \\   
 $\rm Log(\rho_{ign})$          & 8.194    & 8.748     &  8.900  & 8.448   & 9.032   & 8.305   & 8.501    \\   
 $\rm \psi_{ign}$               & 5.77     & 10.83     &  12.36  & 8.087   & 13.26   & 6.154   & 7.748    \\      
 $\rm M_{ign}$                  & 0.948    & 0.340     & 0.069   & 0.457   & 0.000   & 0.404   & 0.000    \\   
 $\rm M_{SiS}$                  & 1.32370  & 1.28943   & 1.33520 & 1.41943 & 1.44115 & 1.48123 & 1.50483  \\   
 $\rm M_{ONe}$                  & 1.35702  & 1.39884   & 1.46271 & 1.65755 & 1.84782 & 2.08227 & 2.63457  \\   
 $\rm M_{CO}$                   & 1.36596  & 1.41091   & 1.47625 & 1.69221 & 1.90364 & 2.16669 & 2.76339  \\   
 $\rm M_{He}$                   & 1.57763  & 1.63765   & 2.71881 & 3.10040 & 3.48811 & 3.90071 & 4.77717  \\   
 $\rm M_{CE}$                   & 1.57787  & 1.63842   & 2.73420 & 3.16664 & 3.59772 & 4.02512 & 4.97346  \\   
 $\rm M_{tot}$                  & 8.754    & 9.006     & 9.429   & 10.2380 & 11.0857 & 11.9090  &13.6102   \\   
\cutinhead{ Quantities at Presupernova Stage}
%%%%  Model                       197300    255700     104700     171600    3100     38900    25700
 $\rm M_{Fe}$                   & 1.263    & 1.265     & 1.211   & 1.316   & 1.333   & 1.456   & 1.398    \\   
 $\rm Log(T_{c})$               & 9.684    & 9.723     & 9.720   & 9.755   & 9.804   & 9.755   & 9.772    \\   
 $\rm Log(\rho_{c})$            & 9.669    & 9.654     & 9.521   & 9.460   & 9.258   & 9.274   & 9.271    \\   
 $\rm \psi_{c}$                 & 14.79    & 12.92     & 11.59   & 10.07   & 7.458   & 8.532   & 8.177    \\      
 $\rm Y_{e,c}$                  & 0.437    & 0.438     & 0.438   & 0.436   & 0.440   & 0.438   & 0.438         
\enddata 
\end{deluxetable*} 



==> tabyieldsNI007.tex <==
\startlongtable
\floattable
\begin{deluxetable}{lcccccc}
%\tabletypesize{\scriptsize}
%\setlength{\tabcolsep}{0.02in}
\tablecolumns{7}
%\tablewidth{626.20622pt}
\tablecaption{Ejected Masses at $\rm 2.5\cdot 10^4~s$ \label{tabyields}}
\tablehead{$\rm Isotope$ & $\rm 9.22~M_\odot$ & $\rm 10~M_\odot$ & $\rm 11~M_\odot$ & $\rm 12~M_\odot$ & $\rm 13~M_\odot$ & $\rm 15~M_\odot$}
\startdata
$\rm^{1}H   $ &   4.6758E+00 & 5.0550E+00 & 5.4726E+00 & 5.8842E+00 & 6.2723E+00 & 7.0091E+00 \\             
$\rm^{2}H   $ &   1.2423E-06 & 1.3362E-06 & 2.7773E-06 & 3.1539E-06 & 3.6321E-06 & 3.4408E-06 \\           
$\rm^{3}H   $ &   7.5762E-22 & 4.8001E-16 & 3.7366E-16 & 3.5642E-33 & 1.0151E-30 & 6.7190E-27 \\           
$\rm^{3}He  $ &   3.0811E-04 & 3.2296E-04 & 3.3389E-04 & 3.4690E-04 & 3.6025E-04 & 3.9009E-04 \\           
$\rm^{4}He  $ &   3.0605E+00 & 3.3310E+00 & 3.6808E+00 & 4.0286E+00 & 4.3419E+00 & 4.9406E+00 \\           
$\rm^{6}Li  $ &   2.5150E-11 & 2.7051E-11 & 5.6228E-11 & 6.3853E-11 & 7.3535E-11 & 6.9662E-11 \\           
$\rm^{7}Li  $ &   3.5727E-10 & 3.8455E-10 & 8.0077E-10 & 9.0700E-10 & 1.0445E-09 & 9.8952E-10 \\           
$\rm^{7}Be  $ &   2.5805E-14 & 2.3128E-11 & 4.6408E-10 & 4.8469E-22 & 2.1430E-20 & 1.4975E-17 \\           
$\rm^{9}Be  $ &   1.4844E-11 & 1.7597E-11 & 1.9878E-11 & 2.1469E-11 & 2.3268E-11 & 2.4634E-11 \\           
$\rm^{10}Be $ &   1.7661E-18 & 2.9197E-19 & 1.9306E-19 & 9.6660E-40 & 1.0444E-39 & 1.2071E-39 \\           
$\rm^{10}B  $ &   1.7214E-10 & 2.0570E-10 & 2.2212E-10 & 2.3666E-10 & 2.5033E-10 & 2.7643E-10 \\           
$\rm^{11}B  $ &   5.4881E-09 & 6.0971E-09 & 6.6036E-09 & 7.0917E-09 & 7.5589E-09 & 8.4702E-09 \\           
$\rm^{12}C  $ &   2.7651E-02 & 3.6903E-02 & 5.4733E-02 & 7.9710E-02 & 1.1326E-01 & 1.7461E-01 \\           
$\rm^{13}C  $ &   4.3668E-04 & 4.9003E-04 & 5.3509E-04 & 5.8725E-04 & 6.4081E-04 & 7.2933E-04 \\           
$\rm^{14}C  $ &   2.7811E-08 & 5.4103E-08 & 1.5229E-08 & 2.2410E-08 & 8.8157E-08 & 2.0197E-07 \\           
$\rm^{13}N  $ &   6.7753E-15 & 2.3873E-15 & 1.8533E-14 & 5.3464E-14 & 5.7210E-14 & 3.6098E-14 \\           
$\rm^{14}N  $ &   2.4452E-02 & 2.4141E-02 & 2.9164E-02 & 3.2127E-02 & 3.4300E-02 & 3.7577E-02 \\           
$\rm^{15}N  $ &   5.2783E-06 & 6.2059E-06 & 5.8130E-06 & 6.2593E-06 & 6.6118E-06 & 7.3764E-06 \\           
$\rm^{16}N  $ &   3.8018E-30 & 1.4585E-31 & 6.2176E-28 & 4.2320E-30 & 5.1761E-27 & 2.9792E-33 \\           
$\rm^{15}O  $ &   1.3235E-21 & 2.7337E-17 & 2.7620E-17 & 3.7233E-17 & 1.5500E-15 & 5.3882E-16 \\           
$\rm^{16}O  $ &   4.8055E-02 & 7.4294E-02 & 1.5758E-01 & 2.2866E-01 & 3.5156E-01 & 5.9481E-01 \\           
$\rm^{17}O  $ &   5.4097E-05 & 5.4178E-05 & 5.5634E-05 & 5.7930E-05 & 5.7043E-05 & 5.7326E-05 \\           
$\rm^{18}O  $ &   1.9470E-04 & 2.7384E-03 & 9.8078E-04 & 7.0057E-04 & 9.3260E-04 & 1.4677E-03 \\           
$\rm^{19}O  $ &   1.2301E-25 & 3.2049E-25 & 4.8739E-21 & 1.1491E-23 & 3.1449E-21 & 1.8962E-27 \\           
$\rm^{17}F  $ &   3.4269E-22 & 1.8867E-24 & 6.3065E-23 & 8.8326E-27 & 1.4790E-24 & 4.6469E-27 \\           
$\rm^{18}F  $ &   7.1406E-11 & 4.2976E-08 & 5.7844E-09 & 3.2255E-09 & 8.4228E-09 & 4.1860E-09 \\           
$\rm^{19}F  $ &   3.2150E-06 & 3.1711E-06 & 3.2536E-06 & 3.4731E-06 & 3.7473E-06 & 4.1927E-06 \\           
$\rm^{20}F  $ &   7.9977E-25 & 5.6514E-25 & 2.0108E-24 & 2.3746E-25 & 1.0332E-21 & 7.3223E-26 \\           
$\rm^{20}Ne $ &   1.1675E-02 & 1.9009E-02 & 3.5053E-02 & 7.8528E-02 & 8.9162E-02 & 2.9002E-01 \\           
$\rm^{21}Ne $ &   4.2647E-05 & 5.0157E-05 & 5.4575E-05 & 7.5797E-05 & 9.4960E-05 & 2.1879E-04 \\           
$\rm^{22}Ne $ &   2.6311E-03 & 3.6438E-03 & 2.9541E-03 & 3.8325E-03 & 5.0114E-03 & 9.1615E-03 \\           
$\rm^{23}Ne $ &   3.6684E-18 & 1.5261E-17 & 5.2785E-17 & 7.7697E-18 & 4.3672E-15 & 1.0989E-19 \\           
$\rm^{21}Na $ &   9.0210E-18 & 3.7789E-17 & 1.3938E-16 & 1.8930E-17 & 2.2682E-16 & 2.4240E-21 \\           
$\rm^{22}Na $ &   1.8750E-08 & 2.8603E-08 & 3.8205E-08 & 2.2876E-07 & 2.3541E-07 & 1.0221E-06 \\           
$\rm^{23}Na $ &   5.6381E-04 & 6.4895E-04 & 6.7919E-04 & 8.6961E-04 & 1.2948E-03 & 3.7936E-03 \\           
$\rm^{24}Na $ &   3.6171E-08 & 3.1020E-08 & 2.6988E-09 & 1.8456E-08 & 4.5289E-08 & 3.6129E-07 \\           
$\rm^{23}Mg $ &   1.7170E-17 & 9.1369E-17 & 2.4084E-16 & 7.6404E-17 & 7.6902E-14 & 5.3389E-14 \\           
$\rm^{24}Mg $ &   5.0809E-03 & 7.8729E-03 & 2.7018E-02 & 3.8297E-02 & 5.1547E-02 & 8.8128E-02 \\           
$\rm^{25}Mg $ &   5.8413E-04 & 8.0429E-04 & 1.6962E-03 & 2.9684E-03 & 3.3399E-03 & 8.2973E-03 \\           
$\rm^{26}Mg $ &   9.0947E-04 & 1.1796E-03 & 1.8271E-03 & 3.1698E-03 & 3.4287E-03 & 8.3621E-03 \\           
$\rm^{27}Mg $ &   6.4071E-15 & 5.0506E-14 & 1.5113E-14 & 6.3495E-14 & 2.2675E-11 & 1.5641E-14 \\           
$\rm^{25}Al $ &   1.5195E-18 & 5.7726E-20 & 5.6904E-19 & 4.3594E-19 & 4.9295E-18 & 1.0693E-21 \\           
$\rm^{26}Al $ &   2.6652E-06 & 5.2074E-06 & 1.5387E-05 & 3.1272E-05 & 2.5040E-05 & 8.3182E-05 \\           
$\rm^{27}Al $ &   5.3350E-04 & 8.4107E-04 & 2.8805E-03 & 4.0425E-03 & 5.8592E-03 & 9.3676E-03 \\           
$\rm^{28}Al $ &   3.3686E-16 & 1.8411E-14 & 1.2209E-14 & 1.6189E-13 & 1.0429E-10 & 2.4681E-11 \\           
$\rm^{27}Si $ &   1.9359E-22 & 7.0198E-20 & 3.4703E-18 & 1.6946E-18 & 2.4832E-14 & 1.9359E-14 \\           
$\rm^{28}Si $ &   1.1218E-02 & 2.0415E-02 & 4.2969E-02 & 5.6178E-02 & 9.5674E-02 & 1.0953E-01 \\           
$\rm^{29}Si $ &   3.0333E-04 & 4.7386E-04 & 1.9837E-03 & 2.3388E-03 & 3.7150E-03 & 4.1090E-03 \\           
$\rm^{30}Si $ &   2.5698E-04 & 5.2413E-04 & 2.6674E-03 & 2.7305E-03 & 5.4616E-03 & 4.8362E-03 \\           
$\rm^{31}Si $ &   7.4173E-10 & 2.9594E-09 & 1.6268E-08 & 1.9627E-08 & 3.8702E-08 & 1.2930E-07 \\           
$\rm^{32}Si $ &   1.9599E-10 & 4.1728E-10 & 1.7022E-08 & 9.3552E-09 & 2.3476E-08 & 2.3220E-08 \\           
$\rm^{29}P  $ &   3.2696E-21 & 4.8094E-22 & 7.1248E-22 & 7.9198E-23 & 2.7038E-20 & 6.4583E-23 \\           
$\rm^{30}P  $ &   1.0818E-16 & 1.4838E-13 & 1.8084E-13 & 2.6224E-13 & 4.9615E-11 & 6.2495E-12 \\           
$\rm^{31}P  $ &   6.6826E-05 & 1.4584E-04 & 5.2837E-04 & 4.8063E-04 & 1.3169E-03 & 9.1697E-04 \\           
$\rm^{32}P  $ &   2.4533E-08 & 9.1148E-08 & 1.1072E-06 & 1.2300E-06 & 3.3510E-06 & 2.7591E-06 \\           
$\rm^{33}P  $ &   1.6431E-08 & 6.0784E-08 & 4.0613E-07 & 4.1477E-07 & 1.0071E-06 & 8.4029E-07 \\           
$\rm^{34}P  $ &   4.8144E-24 & 1.8971E-24 & 6.0519E-23 & 4.7087E-23 & 7.7311E-19 & 4.2050E-19 \\           
$\rm^{31}S  $ &   9.2194E-29 & 5.8417E-24 & 4.2618E-22 & 1.5808E-22 & 2.6854E-17 & 2.3891E-17 \\           
$\rm^{32}S  $ &   5.6094E-03 & 9.7470E-03 & 1.4751E-02 & 2.0676E-02 & 3.2052E-02 & 3.9790E-02 \\           
$\rm^{33}S  $ &   3.3120E-05 & 7.8529E-05 & 1.2430E-04 & 1.7144E-04 & 3.0517E-04 & 3.1812E-04 \\           
$\rm^{34}S  $ &   2.0568E-04 & 5.7837E-04 & 8.8799E-04 & 1.2540E-03 & 2.2570E-03 & 2.1916E-03 \\           
$\rm^{35}S  $ &   2.8062E-08 & 1.1968E-07 & 1.0336E-06 & 4.9299E-07 & 4.3798E-06 & 1.3777E-06 \\           
$\rm^{36}S  $ &   5.7513E-07 & 6.6469E-07 & 1.9077E-06 & 1.2682E-06 & 5.0769E-06 & 2.8162E-06 \\           
$\rm^{37}S  $ &   1.5642E-20 & 1.9448E-19 & 3.0568E-20 & 9.4104E-21 & 8.6710E-17 & 1.1529E-20 \\           
$\rm^{33}Cl $ &   2.9675E-22 & 1.3806E-24 & 3.3096E-24 & 9.6377E-25 & 1.7453E-23 & 1.5195E-26 \\           
$\rm^{34}Cl $ &   1.8579E-23 & 2.4123E-26 & 6.2131E-26 & 1.0951E-26 & 1.5450E-21 & 2.5785E-21 \\           
$\rm^{35}Cl $ &   5.4820E-05 & 8.2805E-05 & 1.1312E-04 & 1.2381E-04 & 2.6848E-04 & 2.0338E-04 \\           
$\rm^{36}Cl $ &   9.5028E-08 & 2.6727E-07 & 9.1420E-07 & 7.6896E-07 & 3.3896E-06 & 1.7395E-06 \\           
$\rm^{37}Cl $ &   1.7510E-05 & 1.9679E-05 & 2.3209E-05 & 2.7193E-05 & 3.2719E-05 & 4.5875E-05 \\           
$\rm^{38}Cl $ &   2.7666E-13 & 4.3818E-13 & 4.2430E-13 & 1.0857E-12 & 5.7297E-12 & 1.4707E-11 \\           
$\rm^{36}Ar $ &   1.1089E-03 & 1.8282E-03 & 2.5960E-03 & 3.6129E-03 & 5.0918E-03 & 6.6018E-03 \\           
$\rm^{37}Ar $ &   9.2179E-07 & 3.2020E-06 & 3.7945E-06 & 5.7437E-06 & 9.2109E-06 & 1.1489E-05 \\           
$\rm^{38}Ar $ &   1.2296E-04 & 2.7042E-04 & 3.3948E-04 & 4.5069E-04 & 7.0354E-04 & 8.0502E-04 \\           
$\rm^{39}Ar $ &   6.5043E-08 & 1.3063E-07 & 3.2235E-07 & 5.5508E-07 & 7.7296E-07 & 1.4666E-06 \\           
$\rm^{40}Ar $ &   1.9152E-07 & 2.3218E-07 & 3.2658E-07 & 4.4016E-07 & 5.2363E-07 & 7.2122E-07 \\           
$\rm^{41}Ar $ &   1.1506E-11 & 7.4178E-12 & 5.5285E-12 & 1.7661E-11 & 4.4620E-11 & 2.0955E-10 \\           
$\rm^{37}K  $ &   8.0646E-28 & 5.0971E-33 & 3.7840E-33 & 1.1576E-33 & 1.1526E-32 & 4.4047E-34 \\           
$\rm^{38}K  $ &   1.3264E-17 & 9.6610E-15 & 2.4265E-15 & 2.5977E-15 & 2.3378E-14 & 1.6733E-14 \\           
$\rm^{39}K  $ &   2.5897E-05 & 3.5999E-05 & 4.1995E-05 & 5.0898E-05 & 6.3578E-05 & 7.8950E-05 \\           
$\rm^{40}K  $ &   7.4013E-08 & 1.0058E-07 & 1.6390E-07 & 2.2468E-07 & 3.7667E-07 & 5.9376E-07 \\           
$\rm^{41}K  $ &   1.7407E-06 & 1.9017E-06 & 2.1364E-06 & 2.4156E-06 & 2.6525E-06 & 3.4532E-06 \\           
$\rm^{42}K  $ &   4.7916E-10 & 5.1587E-10 & 4.8662E-10 & 3.8446E-09 & 2.0201E-09 & 3.4300E-08 \\           
$\rm^{40}Ca $ &   1.1212E-03 & 1.7597E-03 & 2.4455E-03 & 3.2849E-03 & 4.3986E-03 & 5.7402E-03 \\           
$\rm^{41}Ca $ &   6.1817E-07 & 1.1660E-06 & 1.6014E-06 & 2.2308E-06 & 2.8903E-06 & 4.8402E-06 \\           
$\rm^{42}Ca $ &   4.8824E-06 & 9.3416E-06 & 1.1660E-05 & 1.5110E-05 & 2.0441E-05 & 2.8913E-05 \\           
$\rm^{43}Ca $ &   8.6961E-07 & 1.0682E-06 & 1.4382E-06 & 1.8226E-06 & 2.1681E-06 & 3.8183E-06 \\           
$\rm^{44}Ca $ &   1.1914E-05 & 1.3105E-05 & 1.4975E-05 & 1.6933E-05 & 1.8956E-05 & 2.4321E-05 \\           
$\rm^{45}Ca $ &   8.7525E-09 & 9.0277E-09 & 6.1351E-08 & 1.4886E-07 & 3.7436E-07 & 4.8672E-07 \\           
$\rm^{46}Ca $ &   2.9356E-08 & 4.2805E-08 & 7.8043E-08 & 1.0319E-07 & 2.4824E-07 & 1.4624E-07 \\           
$\rm^{47}Ca $ &   9.7176E-11 & 5.2856E-11 & 1.1974E-10 & 7.5045E-10 & 1.1219E-09 & 2.9825E-09 \\           
$\rm^{48}Ca $ &   1.1369E-06 & 1.2350E-06 & 1.3566E-06 & 1.4826E-06 & 1.5949E-06 & 1.8557E-06 \\           
$\rm^{49}Ca $ &   2.3685E-19 & 1.8911E-18 & 4.2564E-19 & 2.8026E-19 & 4.4358E-17 & 6.5798E-19 \\           
$\rm^{41}Sc $ &   1.5783E-35 & 1.4906E-44 & 1.3813E-44 & 1.5372E-44 & 1.8884E-44 & 2.2468E-44 \\           
$\rm^{42}Sc $ &   1.1283E-30 & 2.4893E-38 & 7.1411E-40 & 5.6740E-42 & 7.3924E-37 & 2.3762E-36 \\           
$\rm^{43}Sc $ &   2.8575E-08 & 5.1812E-08 & 7.0109E-08 & 6.7387E-08 & 3.1103E-08 & 3.1942E-08 \\           
$\rm^{44}Sc $ &   2.0855E-10 & 7.4616E-10 & 1.2065E-09 & 1.8022E-09 & 2.3254E-09 & 5.0688E-09 \\           
$\rm^{45}Sc $ &   4.5061E-07 & 5.4829E-07 & 7.8712E-07 & 9.2542E-07 & 1.2161E-06 & 1.7730E-06 \\           
$\rm^{46}Sc $ &   5.2486E-09 & 7.0962E-09 & 2.5481E-08 & 7.0997E-08 & 1.2811E-07 & 2.3156E-07 \\           
$\rm^{47}Sc $ &   1.9446E-09 & 1.8635E-09 & 3.9259E-09 & 1.4664E-08 & 1.3665E-08 & 5.8944E-08 \\           
$\rm^{48}Sc $ &   4.3756E-10 & 4.1966E-10 & 7.8319E-10 & 3.4768E-09 & 1.5202E-09 & 1.7128E-08 \\           
$\rm^{49}Sc $ &   3.4832E-13 & 4.9919E-13 & 1.3754E-12 & 3.0317E-12 & 2.1351E-12 & 3.0784E-11 \\           
$\rm^{44}Ti $ &   2.8480E-06 & 4.7651E-06 & 5.5771E-06 & 5.7005E-06 & 3.9053E-06 & 4.6907E-06 \\           
$\rm^{45}Ti $ &   7.1426E-09 & 1.0792E-08 & 1.3152E-08 & 1.5763E-08 & 1.5531E-08 & 2.2965E-08 \\           
$\rm^{46}Ti $ &   2.8333E-06 & 4.5073E-06 & 5.9208E-06 & 7.1269E-06 & 8.9054E-06 & 1.2265E-05 \\           
$\rm^{47}Ti $ &   1.9641E-06 & 2.2464E-06 & 2.6475E-06 & 2.9191E-06 & 3.2590E-06 & 3.9754E-06 \\           
$\rm^{48}Ti $ &   1.8270E-05 & 1.9874E-05 & 2.2003E-05 & 2.3986E-05 & 2.5996E-05 & 2.9811E-05 \\           
$\rm^{49}Ti $ &   1.4762E-06 & 1.6255E-06 & 1.9038E-06 & 2.1917E-06 & 2.5014E-06 & 3.2227E-06 \\           
$\rm^{50}Ti $ &   1.4538E-06 & 1.6339E-06 & 2.0452E-06 & 2.4629E-06 & 2.9448E-06 & 4.2319E-06 \\           
$\rm^{51}Ti $ &   4.9874E-17 & 1.4795E-16 & 7.1924E-17 & 3.7077E-16 & 5.9595E-14 & 1.6622E-17 \\           
$\rm^{45}V  $ &   1.0173E-43 & 1.4389E-44 & 1.7328E-44 & 1.9654E-44 & 1.4465E-43 & 5.5019E-44 \\           
$\rm^{46}V  $ &   4.1943E-45 & 8.3539E-45 & 1.0071E-44 & 1.1412E-44 & 6.7669E-42 & 1.1329E-41 \\           
$\rm^{47}V  $ &   2.7985E-11 & 4.9583E-11 & 6.3629E-11 & 6.1005E-11 & 4.0846E-11 & 4.8602E-11 \\           
$\rm^{48}V  $ &   2.2694E-08 & 3.8758E-08 & 5.1603E-08 & 6.2005E-08 & 7.9119E-08 & 1.0541E-07 \\           
$\rm^{49}V  $ &   1.5373E-06 & 1.7758E-06 & 2.7232E-06 & 3.6131E-06 & 5.5810E-06 & 7.3381E-06 \\           
$\rm^{50}V  $ &   9.7472E-09 & 1.4859E-08 & 2.7714E-08 & 3.7753E-08 & 6.7469E-08 & 8.9528E-08 \\           
$\rm^{51}V  $ &   2.5381E-06 & 2.7669E-06 & 3.1040E-06 & 3.4029E-06 & 3.7529E-06 & 4.3585E-06 \\           
$\rm^{52}V  $ &   1.8645E-17 & 8.0168E-17 & 6.7932E-17 & 2.1478E-16 & 4.5943E-14 & 6.0760E-15 \\           
$\rm^{48}Cr $ &   1.9927E-05 & 3.1831E-05 & 4.1415E-05 & 4.6256E-05 & 5.6340E-05 & 6.7161E-05 \\           
$\rm^{49}Cr $ &   2.9631E-09 & 3.6914E-09 & 5.5571E-09 & 7.2974E-09 & 1.1375E-08 & 1.5039E-08 \\           
$\rm^{50}Cr $ &   2.3542E-05 & 1.9948E-05 & 3.4550E-05 & 4.5081E-05 & 7.6983E-05 & 1.2031E-04 \\           
$\rm^{51}Cr $ &   4.5761E-06 & 4.2267E-06 & 7.1207E-06 & 9.7739E-06 & 1.5740E-05 & 2.1100E-05 \\           
$\rm^{52}Cr $ &   1.1104E-04 & 1.2219E-04 & 1.3980E-04 & 1.5192E-04 & 1.7281E-04 & 1.9075E-04 \\           
$\rm^{53}Cr $ &   1.2638E-05 & 1.3730E-05 & 1.5181E-05 & 1.6612E-05 & 1.8011E-05 & 2.0966E-05 \\           
$\rm^{54}Cr $ &   3.5006E-06 & 3.9630E-06 & 5.0048E-06 & 6.0655E-06 & 7.4179E-06 & 1.0962E-05 \\           
$\rm^{55}Cr $ &   3.7380E-17 & 9.3991E-17 & 7.3668E-17 & 2.2325E-16 & 1.0622E-13 & 1.8200E-18 \\           
$\rm^{50}Mn $ &   2.7896E-45 & 5.6328E-45 & 6.7850E-45 & 7.6971E-45 & 9.2335E-45 & 1.1211E-44 \\           
$\rm^{51}Mn $ &   1.2260E-08 & 1.1852E-08 & 1.9630E-08 & 2.6974E-08 & 4.3627E-08 & 5.9812E-08 \\           
$\rm^{52}Mn $ &   4.8525E-05 & 7.8573E-05 & 1.1698E-04 & 1.4252E-04 & 2.2776E-04 & 2.8557E-04 \\           
$\rm^{53}Mn $ &   3.1468E-05 & 3.6334E-05 & 5.8002E-05 & 7.7913E-05 & 1.2606E-04 & 1.6291E-04 \\           
$\rm^{54}Mn $ &   7.2374E-09 & 2.1554E-08 & 6.3528E-08 & 8.1462E-08 & 1.4833E-07 & 1.6143E-07 \\           
$\rm^{55}Mn $ &   8.7178E-05 & 9.4752E-05 & 1.0460E-04 & 1.1421E-04 & 1.2346E-04 & 1.4263E-04 \\           
$\rm^{56}Mn $ &   3.9803E-10 & 1.8351E-09 & 2.5389E-09 & 7.2585E-09 & 7.5354E-09 & 1.9713E-08 \\           
$\rm^{57}Mn $ &   6.8692E-23 & 4.1748E-21 & 4.2709E-20 & 2.8315E-18 & 3.1343E-16 & 5.5460E-18 \\           
$\rm^{52}Fe $ &   1.3580E-04 & 2.2044E-04 & 3.2806E-04 & 3.9945E-04 & 6.3802E-04 & 7.9962E-04 \\           
$\rm^{53}Fe $ &   2.2707E-17 & 2.0197E-14 & 2.6534E-14 & 2.5817E-14 & 1.7087E-13 & 1.0834E-13 \\           
$\rm^{54}Fe $ &   2.0027E-03 & 1.7956E-03 & 2.9913E-03 & 4.0755E-03 & 6.6620E-03 & 9.7541E-03 \\           
$\rm^{55}Fe $ &   3.3156E-05 & 3.4497E-05 & 5.7652E-05 & 8.0466E-05 & 1.3250E-04 & 1.6834E-04 \\           
$\rm^{56}Fe $ &   9.3929E-03 & 1.0205E-02 & 1.1223E-02 & 1.2207E-02 & 1.3185E-02 & 1.5039E-02 \\           
$\rm^{57}Fe $ &   2.2685E-04 & 2.4896E-04 & 2.8886E-04 & 3.2951E-04 & 3.7298E-04 & 4.8761E-04 \\           
$\rm^{58}Fe $ &   3.7352E-05 & 5.1147E-05 & 9.9319E-05 & 1.4076E-04 & 2.1403E-04 & 3.7795E-04 \\           
$\rm^{59}Fe $ &   1.9694E-07 & 3.1119E-07 & 5.4301E-07 & 6.8852E-06 & 6.7279E-06 & 1.4568E-05 \\           
$\rm^{60}Fe $ &   1.2094E-07 & 3.7961E-07 & 1.3572E-06 & 2.2052E-06 & 6.2122E-06 & 3.3987E-06 \\           
$\rm^{61}Fe $ &   1.7599E-17 & 1.5776E-16 & 7.5776E-17 & 2.3414E-17 & 1.2781E-14 & 2.5756E-19 \\           
$\rm^{54}Co $ &   1.9121E-45 & 3.8609E-45 & 4.6508E-45 & 5.2761E-45 & 6.3292E-45 & 7.6846E-45 \\           
$\rm^{55}Co $ &   1.5000E-04 & 1.4432E-04 & 2.2778E-04 & 3.2721E-04 & 5.1992E-04 & 6.9529E-04 \\           
$\rm^{56}Co $ &   1.3378E-06 & 1.3123E-06 & 1.8817E-06 & 2.2083E-06 & 2.9079E-06 & 4.1922E-06 \\           
$\rm^{57}Co $ &   1.5047E-04 & 1.9802E-04 & 1.8515E-04 & 1.6840E-04 & 1.7084E-04 & 1.3789E-04 \\           
$\rm^{58}Co $ &   1.9701E-08 & 1.6937E-07 & 6.5498E-07 & 1.0385E-06 & 1.6274E-06 & 2.0502E-06 \\           
$\rm^{59}Co $ &   3.6130E-05 & 4.4922E-05 & 7.2536E-05 & 9.1920E-05 & 1.2371E-04 & 2.1757E-04 \\           
$\rm^{60}Co $ &   1.4363E-07 & 4.1280E-07 & 9.1859E-07 & 4.4312E-06 & 4.9808E-06 & 1.0954E-05 \\           
$\rm^{61}Co $ &   6.1228E-09 & 1.4088E-08 & 1.8885E-08 & 4.7726E-08 & 4.9217E-08 & 3.6728E-07 \\           
$\rm^{56}Ni $ &   4.7810E-02 & 7.0000E-02 & 7.0000E-02 & 7.0000E-02 & 7.0000E-02 & 7.0000E-02 \\           
$\rm^{57}Ni $ &   2.6241E-03 & 3.4473E-03 & 3.1934E-03 & 2.8827E-03 & 2.8827E-03 & 2.2930E-03 \\           
$\rm^{58}Ni $ &   9.1919E-03 & 1.1529E-02 & 1.0705E-02 & 8.5597E-03 & 1.0545E-02 & 6.5266E-03 \\           
$\rm^{59}Ni $ &   1.6798E-04 & 2.0557E-04 & 1.9299E-04 & 1.5988E-04 & 1.4907E-04 & 1.0525E-04 \\           
$\rm^{60}Ni $ &   1.0092E-03 & 1.5187E-03 & 1.6105E-03 & 1.5005E-03 & 1.2384E-03 & 1.2326E-03 \\           
$\rm^{61}Ni $ &   4.5831E-05 & 6.5424E-05 & 7.1510E-05 & 6.8298E-05 & 7.0480E-05 & 8.2712E-05 \\           
$\rm^{62}Ni $ &   5.6222E-05 & 7.8477E-05 & 9.9263E-05 & 1.0750E-04 & 1.3939E-04 & 1.7824E-04 \\           
$\rm^{63}Ni $ &   8.2361E-07 & 2.3386E-06 & 7.3613E-06 & 1.2519E-05 & 1.7901E-05 & 2.5519E-05 \\           
$\rm^{64}Ni $ &   9.2769E-06 & 1.1763E-05 & 1.9007E-05 & 2.6757E-05 & 3.6471E-05 & 4.4718E-05 \\           
$\rm^{65}Ni $ &   4.5876E-09 & 1.5463E-09 & 1.1666E-09 & 3.6727E-09 & 1.6962E-08 & 2.2069E-08 \\           
$\rm^{57}Cu $ &   2.3962E-45 & 4.8384E-45 & 5.8282E-45 & 6.6118E-45 & 7.9315E-45 & 9.6300E-45 \\           
$\rm^{58}Cu $ &   3.1178E-44 & 1.0109E-36 & 1.9802E-35 & 9.9990E-36 & 1.0053E-32 & 9.4990E-33 \\           
$\rm^{59}Cu $ &   4.3036E-25 & 8.7369E-22 & 1.3007E-22 & 1.9323E-22 & 1.4755E-19 & 3.6694E-20 \\           
$\rm^{60}Cu $ &   1.9464E-08 & 3.7551E-08 & 3.7324E-08 & 3.3331E-08 & 2.6089E-08 & 2.3858E-08 \\           
$\rm^{61}Cu $ &   2.8042E-05 & 4.1001E-05 & 4.1199E-05 & 3.3276E-05 & 2.8167E-05 & 2.0276E-05 \\           
$\rm^{62}Cu $ &   1.1498E-06 & 1.5777E-06 & 1.6620E-06 & 1.1978E-06 & 1.2516E-06 & 7.0831E-07 \\           
$\rm^{63}Cu $ &   6.3947E-06 & 7.4511E-06 & 7.8818E-06 & 8.8158E-06 & 1.0141E-05 & 1.5899E-05 \\           
$\rm^{64}Cu $ &   8.5162E-08 & 1.3204E-07 & 1.4733E-07 & 3.2531E-07 & 3.4235E-07 & 9.6541E-07 \\           
$\rm^{65}Cu $ &   3.2830E-06 & 4.0308E-06 & 6.3698E-06 & 8.9955E-06 & 1.1703E-05 & 1.9608E-05 \\           
$\rm^{66}Cu $ &   3.6567E-15 & 9.5292E-15 & 4.4760E-15 & 1.8364E-14 & 2.7360E-12 & 1.0291E-15 \\           
$\rm^{60}Zn $ &   1.2622E-24 & 5.8841E-23 & 2.7326E-23 & 2.8394E-23 & 3.6185E-23 & 5.2074E-23 \\           
$\rm^{61}Zn $ &   7.9428E-27 & 2.5343E-23 & 4.3982E-25 & 1.3081E-24 & 1.6793E-22 & 9.2779E-23 \\           
$\rm^{62}Zn $ &   8.3630E-04 & 1.1862E-03 & 1.2467E-03 & 8.9634E-04 & 9.3515E-04 & 5.2108E-04 \\           
$\rm^{63}Zn $ &   1.6313E-09 & 2.3178E-09 & 2.2614E-09 & 1.5279E-09 & 1.4759E-09 & 7.6343E-10 \\           
$\rm^{64}Zn $ &   9.9509E-06 & 1.2988E-05 & 1.4215E-05 & 1.4885E-05 & 1.4378E-05 & 1.9463E-05 \\           
$\rm^{65}Zn $ &   5.1980E-07 & 8.5303E-07 & 9.8053E-07 & 1.0745E-06 & 1.0158E-06 & 2.0991E-06 \\           
$\rm^{66}Zn $ &   6.1605E-06 & 8.4622E-06 & 1.0052E-05 & 1.3253E-05 & 1.5970E-05 & 2.5007E-05 \\           
$\rm^{67}Zn $ &   8.4195E-07 & 9.3483E-07 & 1.5701E-06 & 2.0935E-06 & 2.6353E-06 & 4.5403E-06 \\           
$\rm^{68}Zn $ &   3.8882E-06 & 4.5184E-06 & 7.4412E-06 & 9.4092E-06 & 1.3057E-05 & 1.7874E-05 \\           
$\rm^{69}Zn $ &   1.9392E-10 & 1.0464E-10 & 1.4288E-10 & 3.4045E-10 & 7.7626E-10 & 3.1014E-09 \\           
$\rm^{70}Zn $ &   1.4151E-07 & 1.1705E-07 & 1.7110E-07 & 2.4879E-07 & 3.1949E-07 & 4.8628E-07 \\           
$\rm^{71}Zn $ &   4.6210E-22 & 6.9235E-20 & 1.0466E-20 & 1.4585E-18 & 3.1325E-15 & 2.9116E-21 \\           
$\rm^{62}Ga $ &   1.1601E-45 & 2.3424E-45 & 2.8217E-45 & 3.2011E-45 & 3.8400E-45 & 4.6624E-45 \\           
$\rm^{63}Ga $ &   1.3322E-37 & 4.5119E-32 & 1.4560E-33 & 1.6324E-32 & 4.8808E-29 & 1.3010E-30 \\           
$\rm^{64}Ga $ &   2.2176E-27 & 8.4707E-25 & 1.3746E-28 & 2.6225E-27 & 2.9535E-25 & 2.1720E-25 \\           
$\rm^{65}Ga $ &   7.8737E-14 & 1.8457E-13 & 1.8544E-13 & 1.4441E-13 & 1.0885E-13 & 8.5527E-14 \\           
$\rm^{66}Ga $ &   3.5393E-06 & 5.5101E-06 & 6.4271E-06 & 4.4497E-06 & 4.1536E-06 & 2.3931E-06 \\           
$\rm^{67}Ga $ &   2.9680E-08 & 3.7593E-08 & 4.1381E-08 & 3.6142E-08 & 3.3063E-08 & 3.9685E-08 \\           
$\rm^{68}Ga $ &   1.0779E-10 & 1.0778E-10 & 9.9906E-11 & 1.7631E-10 & 1.8345E-10 & 4.3049E-10 \\           
$\rm^{69}Ga $ &   4.8993E-07 & 6.0946E-07 & 9.3487E-07 & 1.2199E-06 & 1.4532E-06 & 2.3587E-06 \\           
$\rm^{70}Ga $ &   1.0337E-13 & 5.2962E-13 & 9.6163E-13 & 1.2581E-12 & 1.0963E-11 & 3.0219E-12 \\           
$\rm^{71}Ga $ &   3.3334E-07 & 3.5461E-07 & 4.8371E-07 & 6.6704E-07 & 8.0185E-07 & 1.3630E-06 \\           
$\rm^{72}Ga $ &   8.3083E-09 & 2.2210E-09 & 1.2078E-09 & 4.2881E-09 & 7.8376E-09 & 1.9180E-08 \\           
$\rm^{64}Ge $ &   1.8577E-37 & 1.2738E-33 & 1.0082E-33 & 2.9586E-35 & 1.0103E-33 & 5.2879E-34 \\           
$\rm^{65}Ge $ &   1.4370E-43 & 1.1397E-35 & 8.5749E-37 & 2.1548E-36 & 2.0853E-33 & 3.6905E-33 \\           
$\rm^{66}Ge $ &   6.8673E-06 & 1.0729E-05 & 1.2480E-05 & 8.6438E-06 & 8.0565E-06 & 4.6396E-06 \\           
$\rm^{67}Ge $ &   3.0999E-14 & 5.9780E-14 & 6.6405E-14 & 4.2450E-14 & 3.6506E-14 & 1.9643E-14 \\           
$\rm^{68}Ge $ &   1.7446E-08 & 2.3344E-08 & 2.2528E-08 & 1.4502E-08 & 1.6979E-08 & 1.2555E-08 \\           
$\rm^{69}Ge $ &   5.9376E-10 & 8.3364E-10 & 4.2652E-10 & 1.0325E-09 & 1.0021E-09 & 2.3662E-09 \\           
$\rm^{70}Ge $ &   6.6209E-07 & 9.4553E-07 & 1.1466E-06 & 1.4963E-06 & 1.7202E-06 & 2.7569E-06 \\           
$\rm^{71}Ge $ &   2.8373E-08 & 2.8211E-08 & 9.9821E-08 & 1.6379E-07 & 2.0882E-07 & 3.6702E-07 \\           
$\rm^{72}Ge $ &   7.8501E-07 & 1.0185E-06 & 1.4602E-06 & 1.8232E-06 & 2.1951E-06 & 3.0334E-06 \\           
$\rm^{73}Ge $ &   2.0591E-07 & 2.3031E-07 & 3.9178E-07 & 5.0022E-07 & 5.9293E-07 & 8.7946E-07 \\           
$\rm^{74}Ge $ &   9.5125E-07 & 1.1044E-06 & 1.7488E-06 & 2.1565E-06 & 2.8528E-06 & 3.3420E-06 \\           
$\rm^{75}Ge $ &   4.9825E-10 & 2.2758E-10 & 3.4557E-10 & 8.2160E-10 & 1.6328E-09 & 6.9154E-09 \\           
$\rm^{76}Ge $ &   1.6990E-07 & 1.6950E-07 & 2.0147E-07 & 2.4299E-07 & 2.9246E-07 & 3.5669E-07 \\           
$\rm^{77}Ge $ &   3.8909E-10 & 3.2139E-11 & 2.7430E-11 & 1.1217E-10 & 2.1718E-10 & 6.0987E-10 \\           
$\rm^{71}As $ &   7.6703E-11 & 4.0907E-11 & 4.2395E-11 & 6.0056E-11 & 4.5414E-11 & 1.1452E-10 \\           
$\rm^{72}As $ &   1.1458E-10 & 6.4727E-11 & 4.8789E-11 & 8.6594E-11 & 6.9550E-11 & 1.9255E-10 \\           
$\rm^{73}As $ &   6.1986E-09 & 6.2215E-09 & 5.4479E-09 & 8.5075E-09 & 8.7931E-09 & 1.6844E-08 \\           
$\rm^{74}As $ &   1.5251E-09 & 1.0291E-09 & 1.1269E-09 & 1.6911E-09 & 1.6102E-09 & 3.2882E-09 \\           
$\rm^{75}As $ &   1.5189E-07 & 1.7946E-07 & 2.8603E-07 & 3.9806E-07 & 4.5631E-07 & 6.7481E-07 \\           
$\rm^{76}As $ &   4.8010E-09 & 2.8692E-09 & 5.8324E-09 & 1.0688E-08 & 1.4521E-08 & 1.4107E-08 \\           
$\rm^{77}As $ &   2.3001E-08 & 1.9538E-08 & 2.3370E-08 & 5.9587E-08 & 5.2682E-08 & 1.2877E-07 \\           
$\rm^{74}Se $ &   2.1809E-08 & 5.1847E-08 & 3.7281E-08 & 6.1599E-08 & 6.3026E-08 & 1.0163E-07 \\           
$\rm^{75}Se $ &   2.0656E-09 & 3.2780E-09 & 1.8457E-09 & 3.6055E-09 & 3.4456E-09 & 6.7704E-09 \\           
$\rm^{76}Se $ &   1.6429E-07 & 2.6150E-07 & 3.1912E-07 & 3.9498E-07 & 4.2730E-07 & 5.7994E-07 \\           
$\rm^{77}Se $ &   9.5247E-08 & 1.0709E-07 & 1.6280E-07 & 1.8107E-07 & 2.2259E-07 & 2.5024E-07 \\           
$\rm^{78}Se $ &   3.3849E-07 & 4.1270E-07 & 6.6193E-07 & 7.5859E-07 & 8.8446E-07 & 1.0479E-06 \\           
$\rm^{79}Se $ &   1.1500E-08 & 2.4539E-08 & 8.3149E-08 & 1.2033E-07 & 1.4032E-07 & 1.8917E-07 \\           
$\rm^{80}Se $ &   5.8077E-07 & 6.6736E-07 & 9.1681E-07 & 1.0614E-06 & 1.2538E-06 & 1.2772E-06 \\           
$\rm^{81}Se $ &   4.8098E-15 & 3.5457E-14 & 1.0367E-13 & 1.6082E-13 & 2.6248E-12 & 4.0604E-13 \\           
$\rm^{82}Se $ &   1.0252E-07 & 1.0390E-07 & 1.1686E-07 & 1.3876E-07 & 1.7319E-07 & 1.9847E-07 \\           
$\rm^{83}Se $ &   2.2870E-16 & 6.7307E-17 & 4.0455E-16 & 8.3141E-16 & 2.4316E-14 & 4.7419E-15 \\           
$\rm^{75}Br $ &   3.0790E-14 & 2.7128E-14 & 8.6796E-15 & 1.0964E-14 & 9.1901E-15 & 1.5840E-14 \\           
$\rm^{76}Br $ &   3.2991E-12 & 2.5118E-12 & 7.8396E-13 & 2.1535E-12 & 1.5155E-12 & 4.2665E-12 \\           
$\rm^{77}Br $ &   2.1545E-10 & 2.3986E-10 & 8.2007E-11 & 1.6664E-10 & 1.3115E-10 & 2.9818E-10 \\           
$\rm^{78}Br $ &   3.2577E-18 & 3.6296E-16 & 4.6719E-18 & 8.8279E-18 & 4.8390E-16 & 4.2895E-16 \\           
$\rm^{79}Br $ &   8.8304E-08 & 9.4990E-08 & 1.0742E-07 & 1.0974E-07 & 1.2075E-07 & 1.4083E-07 \\           
$\rm^{80}Br $ &   1.1617E-14 & 1.3936E-13 & 5.6969E-14 & 1.3560E-14 & 1.8812E-12 & 3.2670E-14 \\           
$\rm^{81}Br $ &   1.0101E-07 & 1.1670E-07 & 1.6399E-07 & 1.9846E-07 & 2.2821E-07 & 2.4614E-07 \\           
$\rm^{82}Br $ &   1.2652E-09 & 7.3967E-10 & 2.6800E-09 & 6.8734E-09 & 5.4880E-09 & 7.5944E-09 \\           
$\rm^{83}Br $ &   1.2726E-09 & 1.1242E-09 & 2.3666E-09 & 3.6737E-09 & 3.8932E-09 & 8.5207E-09 \\           
$\rm^{78}Kr $ &   3.5773E-09 & 5.8862E-09 & 6.1713E-09 & 7.5132E-09 & 7.9248E-09 & 8.8188E-09 \\           
$\rm^{79}Kr $ &   5.2916E-11 & 1.5469E-10 & 1.7289E-10 & 2.0514E-10 & 2.0198E-10 & 2.4355E-10 \\           
$\rm^{80}Kr $ &   3.1112E-08 & 4.3875E-08 & 5.5573E-08 & 6.2319E-08 & 6.5856E-08 & 8.3729E-08 \\           
$\rm^{81}Kr $ &   2.2405E-09 & 1.7787E-09 & 2.1518E-09 & 3.3229E-09 & 2.5094E-09 & 1.1228E-08 \\           
$\rm^{82}Kr $ &   1.3275E-07 & 1.5977E-07 & 2.1477E-07 & 2.4332E-07 & 2.5971E-07 & 3.2128E-07 \\           
$\rm^{83}Kr $ &   1.1741E-07 & 1.2765E-07 & 1.8704E-07 & 2.2328E-07 & 2.6196E-07 & 2.9958E-07 \\           
$\rm^{84}Kr $ &   5.3822E-07 & 6.0391E-07 & 8.6853E-07 & 9.5145E-07 & 1.0546E-06 & 1.3044E-06 \\           
$\rm^{85}Kr $ &   3.8801E-09 & 1.0503E-08 & 7.8585E-08 & 9.6109E-08 & 1.1096E-07 & 1.4629E-07 \\           
$\rm^{86}Kr $ &   1.7514E-07 & 2.0678E-07 & 3.4960E-07 & 3.6573E-07 & 4.5272E-07 & 4.6276E-07 \\           
$\rm^{87}Kr $ &   4.3110E-13 & 1.8238E-13 & 2.3086E-13 & 3.5864E-13 & 4.4656E-12 & 1.0655E-12 \\           
$\rm^{79}Rb $ &   2.6193E-19 & 5.5378E-18 & 4.3118E-19 & 7.4458E-19 & 3.4480E-18 & 2.4320E-18 \\           
$\rm^{80}Rb $ &   1.6475E-29 & 2.1507E-23 & 2.0306E-24 & 1.0395E-23 & 3.4209E-20 & 1.1507E-20 \\           
$\rm^{81}Rb $ &   1.6952E-13 & 4.7065E-13 & 1.0203E-13 & 1.8056E-13 & 1.6578E-13 & 2.4656E-13 \\           
$\rm^{82}Rb $ &   1.0570E-23 & 1.0164E-19 & 2.7588E-21 & 2.3190E-20 & 2.3877E-17 & 2.2047E-17 \\           
$\rm^{83}Rb $ &   5.9915E-11 & 2.0159E-10 & 2.5154E-10 & 2.8027E-10 & 3.0261E-10 & 3.3766E-10 \\           
$\rm^{84}Rb $ &   1.0992E-11 & 2.4247E-11 & 3.1103E-11 & 3.2857E-11 & 3.4713E-11 & 3.9312E-11 \\           
$\rm^{85}Rb $ &   1.2540E-07 & 1.4140E-07 & 1.7677E-07 & 1.9037E-07 & 2.0825E-07 & 2.4056E-07 \\           
$\rm^{86}Rb $ &   1.0118E-09 & 1.5671E-09 & 8.7724E-09 & 1.6323E-08 & 1.6782E-08 & 2.6928E-08 \\           
$\rm^{87}Rb $ &   5.9080E-08 & 7.5342E-08 & 1.6508E-07 & 1.8268E-07 & 2.6411E-07 & 2.2816E-07 \\           
$\rm^{88}Rb $ &   8.3467E-17 & 7.7150E-16 & 1.6388E-15 & 1.6489E-15 & 1.0371E-13 & 2.4812E-15 \\           
$\rm^{84}Sr $ &   2.5367E-09 & 6.4730E-09 & 5.6308E-09 & 7.9518E-09 & 8.9759E-09 & 9.1477E-09 \\           
$\rm^{85}Sr $ &   3.7021E-11 & 1.9585E-10 & 3.2083E-10 & 4.1970E-10 & 4.4458E-10 & 4.3649E-10 \\           
$\rm^{86}Sr $ &   5.1850E-08 & 6.2316E-08 & 9.7237E-08 & 1.0481E-07 & 1.0904E-07 & 1.5727E-07 \\           
$\rm^{87}Sr $ &   3.2313E-08 & 3.6787E-08 & 5.9854E-08 & 7.0472E-08 & 6.9504E-08 & 1.1785E-07 \\           
$\rm^{88}Sr $ &   3.4039E-07 & 4.0484E-07 & 7.2238E-07 & 7.8819E-07 & 8.8175E-07 & 1.0635E-06 \\           
$\rm^{89}Sr $ &   4.1677E-10 & 7.0856E-10 & 4.9472E-09 & 1.1788E-08 & 1.0276E-08 & 2.0529E-08 \\           
$\rm^{90}Sr $ &   1.8052E-10 & 2.9079E-10 & 3.2613E-09 & 4.3414E-09 & 5.3861E-09 & 4.6955E-09 \\           
$\rm^{91}Sr $ &   1.0210E-12 & 3.5163E-13 & 6.8911E-13 & 1.7310E-12 & 1.3232E-11 & 4.5358E-12 \\           
$\rm^{85}Y  $ &   3.5900E-16 & 5.0174E-15 & 4.7830E-16 & 1.2009E-15 & 2.0477E-15 & 1.8683E-15 \\           
$\rm^{86}Y  $ &   3.5406E-15 & 2.2803E-14 & 7.4563E-15 & 1.3710E-14 & 1.5624E-14 & 1.6705E-14 \\           
$\rm^{87}Y  $ &   1.2986E-12 & 9.2453E-12 & 6.5571E-12 & 9.3070E-12 & 9.9648E-12 & 1.0756E-11 \\           
$\rm^{88}Y  $ &   2.6218E-12 & 1.5272E-11 & 2.0019E-11 & 2.5780E-11 & 2.4941E-11 & 2.8607E-11 \\           
$\rm^{89}Y  $ &   8.7988E-08 & 1.0395E-07 & 1.4308E-07 & 1.5927E-07 & 1.6321E-07 & 2.0697E-07 \\           
$\rm^{90}Y  $ &   6.9429E-11 & 1.5954E-10 & 4.5396E-10 & 1.7080E-09 & 4.9852E-10 & 2.0204E-09 \\           
$\rm^{91}Y  $ &   2.3918E-10 & 4.3546E-10 & 5.5460E-09 & 6.3491E-09 & 7.3615E-09 & 7.3127E-09 \\           
$\rm^{90}Zr $ &   1.0455E-07 & 1.2110E-07 & 1.5304E-07 & 1.6628E-07 & 1.7762E-07 & 2.1338E-07 \\           
$\rm^{91}Zr $ &   2.3043E-08 & 2.5665E-08 & 3.5048E-08 & 3.6726E-08 & 3.9811E-08 & 4.8511E-08 \\           
$\rm^{92}Zr $ &   3.5736E-08 & 4.0114E-08 & 5.3434E-08 & 5.7498E-08 & 6.4215E-08 & 7.3767E-08 \\           
$\rm^{93}Zr $ &   4.1076E-10 & 7.1280E-10 & 2.8758E-09 & 3.7473E-09 & 3.7800E-09 & 6.8914E-09 \\           
$\rm^{94}Zr $ &   3.6514E-08 & 4.0178E-08 & 4.9844E-08 & 5.3795E-08 & 5.9805E-08 & 6.8377E-08 \\           
$\rm^{95}Zr $ &   5.2319E-11 & 7.2603E-11 & 2.9861E-10 & 6.7747E-10 & 8.9675E-10 & 1.8563E-09 \\           
$\rm^{96}Zr $ &   5.9762E-09 & 6.5773E-09 & 8.1290E-09 & 9.1949E-09 & 1.0282E-08 & 1.1270E-08 \\           
$\rm^{97}Zr $ &   1.3925E-13 & 3.0342E-14 & 2.3918E-14 & 7.6886E-14 & 4.7061E-12 & 1.7184E-13 \\           
$\rm^{91}Nb $ &   3.2627E-12 & 2.1556E-11 & 3.5595E-11 & 4.2141E-11 & 4.1385E-11 & 5.1969E-11 \\           
$\rm^{92}Nb $ &   8.4675E-13 & 3.8456E-12 & 5.8068E-12 & 6.6832E-12 & 5.9916E-12 & 7.8858E-12 \\           
$\rm^{93}Nb $ &   1.5159E-08 & 1.6459E-08 & 1.7938E-08 & 1.9389E-08 & 2.0728E-08 & 2.3292E-08 \\           
$\rm^{94}Nb $ &   3.0990E-11 & 1.3897E-11 & 1.8254E-11 & 3.3269E-11 & 4.9903E-11 & 1.1272E-10 \\           
$\rm^{95}Nb $ &   1.0160E-11 & 3.5069E-11 & 1.0813E-10 & 7.3676E-11 & 1.9877E-10 & 2.3045E-10 \\           
$\rm^{96}Nb $ &   1.3137E-12 & 2.7659E-12 & 2.7858E-12 & 3.5656E-12 & 7.2186E-12 & 1.2364E-11 \\           
$\rm^{97}Nb $ &   8.9272E-14 & 2.3152E-13 & 1.2831E-13 & 1.3184E-13 & 6.8219E-13 & 2.2064E-12 \\           
$\rm^{92}Mo $ &   5.8641E-09 & 6.6247E-09 & 7.7347E-09 & 8.4701E-09 & 9.2844E-09 & 1.0715E-08 \\           
$\rm^{93}Mo $ &   7.9438E-12 & 2.1147E-11 & 4.7725E-11 & 5.6314E-11 & 6.4561E-11 & 8.9948E-11 \\           
$\rm^{94}Mo $ &   4.0927E-09 & 4.6330E-09 & 5.3821E-09 & 5.9181E-09 & 6.4171E-09 & 7.4351E-09 \\           
$\rm^{95}Mo $ &   6.6351E-09 & 7.2360E-09 & 7.9775E-09 & 8.6798E-09 & 9.1654E-09 & 1.0438E-08 \\           
$\rm^{96}Mo $ &   7.2324E-09 & 7.9942E-09 & 9.1915E-09 & 1.0069E-08 & 1.0688E-08 & 1.2857E-08 \\           
$\rm^{97}Mo $ &   4.1015E-09 & 4.4793E-09 & 4.9587E-09 & 5.4757E-09 & 5.7804E-09 & 6.9226E-09 \\           
$\rm^{98}Mo $ &   1.0631E-08 & 1.1627E-08 & 1.3089E-08 & 1.4352E-08 & 1.5252E-08 & 1.8405E-08 \\           
$\rm^{132}Xe$ &   3.5335E-08 & 3.8605E-08 & 4.4443E-08 & 4.8085E-08 & 5.2145E-08 & 6.0427E-08 \\           
$\rm^{133}Xe$ &   1.4856E-11 & 1.4693E-11 & 2.5237E-11 & 1.7896E-10 & 8.0201E-11 & 3.9454E-10 \\           
$\rm^{134}Xe$ &   1.3209E-08 & 1.4366E-08 & 1.6184E-08 & 1.7687E-08 & 1.9452E-08 & 2.1838E-08 \\           
$\rm^{135}Xe$ &   2.5247E-12 & 1.4336E-12 & 1.5307E-12 & 4.4271E-12 & 5.0759E-12 & 2.5235E-11 \\           
$\rm^{133}Cs$ &   9.0974E-09 & 9.9211E-09 & 1.0982E-08 & 1.1834E-08 & 1.2871E-08 & 1.4732E-08 \\           
$\rm^{134}Cs$ &   7.5308E-12 & 1.7218E-11 & 4.0461E-11 & 7.3428E-11 & 1.0541E-10 & 2.5222E-10 \\           
$\rm^{135}Cs$ &   7.6729E-11 & 1.6275E-10 & 5.3369E-10 & 7.7141E-10 & 8.7549E-10 & 1.5379E-09 \\           
$\rm^{136}Cs$ &   3.9485E-12 & 7.0735E-12 & 2.2252E-11 & 1.4480E-10 & 9.3027E-11 & 3.6279E-10 \\           
$\rm^{137}Cs$ &   2.3759E-11 & 8.5386E-11 & 6.7744E-10 & 9.9224E-10 & 1.3121E-09 & 1.4036E-09 \\           
$\rm^{138}Cs$ &   5.1614E-19 & 3.8889E-18 & 2.4028E-18 & 3.0245E-17 & 1.1358E-15 & 1.1058E-17 \\           
$\rm^{134}Ba$ &   3.1984E-09 & 3.5205E-09 & 3.9953E-09 & 4.3980E-09 & 4.8241E-09 & 5.7403E-09 \\           
$\rm^{135}Ba$ &   7.5900E-09 & 8.2202E-09 & 8.9519E-09 & 9.6741E-09 & 1.0350E-08 & 1.1707E-08 \\           
$\rm^{136}Ba$ &   9.7697E-09 & 1.0789E-08 & 1.2474E-08 & 1.3735E-08 & 1.5117E-08 & 1.8720E-08 \\           
$\rm^{137}Ba$ &   1.3569E-08 & 1.4810E-08 & 1.6437E-08 & 1.8099E-08 & 1.9371E-08 & 2.3649E-08 \\           
$\rm^{138}Ba$ &   8.7772E-08 & 9.6129E-08 & 1.1016E-07 & 1.2250E-07 & 1.3518E-07 & 1.6559E-07 \\           
$\rm^{139}Ba$ &   1.1701E-14 & 6.0165E-15 & 1.3539E-15 & 1.1166E-14 & 3.9433E-13 & 5.5033E-15 \\           
$\rm^{138}La$ &   8.8564E-12 & 9.6625E-12 & 1.0662E-11 & 1.1565E-11 & 1.2507E-11 & 1.4105E-11 \\           
$\rm^{139}La$ &   1.0227E-08 & 1.1200E-08 & 1.2706E-08 & 1.4158E-08 & 1.5663E-08 & 1.9093E-08 \\           
$\rm^{140}La$ &   3.5018E-13 & 7.4634E-14 & 1.6542E-14 & 1.2587E-13 & 7.3539E-12 & 8.6683E-14 \\           
$\rm^{140}Ce$ &   2.7444E-08 & 2.9929E-08 & 3.3451E-08 & 3.6912E-08 & 4.0361E-08 & 4.7756E-08 \\           
$\rm^{141}Ce$ &   2.2223E-12 & 5.9355E-13 & 4.2013E-13 & 1.4019E-12 & 7.5892E-11 & 1.0293E-11 \\           
$\rm^{141}Pr$ &   4.2707E-09 & 4.6512E-09 & 5.1944E-09 & 5.7174E-09 & 6.0957E-09 & 7.0322E-09 \\           
$\rm^{142}Pr$ &   5.5365E-13 & 9.0732E-14 & 4.9165E-14 & 2.2092E-13 & 4.8494E-12 & 4.3948E-13 \\           
$\rm^{142}Nd$ &   5.9629E-09 & 6.5907E-09 & 7.5667E-09 & 8.4529E-09 & 9.5033E-09 & 1.1348E-08 \\           
$\rm^{143}Nd$ &   2.5719E-09 & 2.7913E-09 & 3.0445E-09 & 3.3028E-09 & 3.5479E-09 & 4.0634E-09 \\           
$\rm^{144}Nd$ &   5.2375E-09 & 5.6941E-09 & 6.2646E-09 & 6.8423E-09 & 7.4261E-09 & 8.5919E-09 \\           
$\rm^{202}Hg$ &   5.2295E-09 & 5.6921E-09 & 6.3973E-09 & 7.1127E-09 & 7.6773E-09 & 9.3406E-09 \\           
$\rm^{203}Hg$ &   3.4365E-12 & 2.3568E-12 & 1.1833E-12 & 5.7036E-12 & 6.8187E-11 & 1.2047E-10 \\           
$\rm^{204}Hg$ &   1.1964E-09 & 1.3029E-09 & 1.4324E-09 & 1.5858E-09 & 1.7571E-09 & 1.9617E-09 \\           
$\rm^{205}Hg$ &   4.6532E-21 & 5.7901E-20 & 2.6851E-20 & 5.5695E-21 & 1.2002E-18 & 6.1592E-22 \\           
$\rm^{203}Tl$ &   2.7602E-09 & 3.0077E-09 & 3.3520E-09 & 3.6814E-09 & 3.9389E-09 & 4.6783E-09 \\           
$\rm^{204}Tl$ &   2.7128E-12 & 5.3998E-12 & 2.2216E-11 & 4.5463E-11 & 4.0681E-11 & 1.5096E-10 \\           
$\rm^{205}Tl$ &   6.6272E-09 & 7.2086E-09 & 7.9334E-09 & 8.6921E-09 & 9.3051E-09 & 1.0782E-08 \\           
$\rm^{206}Tl$ &   4.9024E-20 & 1.2224E-19 & 8.2441E-20 & 7.1406E-20 & 2.4017E-17 & 7.1165E-22 \\           
$\rm^{204}Pb$ &   1.3691E-09 & 1.5031E-09 & 1.7027E-09 & 1.8700E-09 & 2.1892E-09 & 2.5191E-09 \\           
$\rm^{205}Pb$ &   2.3542E-11 & 2.8221E-11 & 4.8578E-11 & 7.1702E-11 & 1.3344E-10 & 2.8824E-10 \\           
$\rm^{206}Pb$ &   1.2578E-08 & 1.3737E-08 & 1.5680E-08 & 1.7309E-08 & 1.9561E-08 & 2.3007E-08 \\           
$\rm^{207}Pb$ &   1.3124E-08 & 1.4187E-08 & 1.5425E-08 & 1.6967E-08 & 1.8124E-08 & 2.1982E-08 \\           
$\rm^{208}Pb$ &   3.7676E-08 & 4.0691E-08 & 4.4559E-08 & 4.8743E-08 & 5.2347E-08 & 6.1776E-08 \\           
$\rm^{209}Pb$ &   2.1274E-16 & 2.1841E-16 & 2.4099E-16 & 1.9698E-15 & 1.1240E-13 & 7.7855E-16 \\           
$\rm^{208}Bi$ &   3.5107E-11 & 6.1163E-11 & 1.2148E-10 & 1.6502E-10 & 2.9724E-10 & 3.0993E-10 \\           
$\rm^{209}Bi$ &   5.0879E-09 & 5.4854E-09 & 5.9526E-09 & 6.4658E-09 & 6.8909E-09 & 7.9884E-09 \\           
\enddata                  
\end{deluxetable}         

